The Intriguing Properties of Model Explanations

Linear approximations to the decision boundary of a complex model have become one of the most popular tools for interpreting predictions. In this paper, we study such linear explanations produced either post-hoc by a few recent methods or generated along with predictions with contextual explanation networks (CENs). We focus on two questions: (i) whether linear explanations are always consistent or can be misleading, and (ii) when integrated into the prediction process, whether and how explanations affect the performance of the model. Our analysis sheds more light on certain properties of explanations produced by different methods and suggests that learning models that explain and predict jointly is often advantageous.

==> figures/imdb-dict-tpc.tex <==
%!TEX root = ../paper.tex

\begin{figure}[t!]
\centering
\includegraphics[width=\textwidth]{imdb-dictionary.pdf}%
\caption{%
The full dictionary learned by CEN$_\mathrm{tpc}$ model: rows correspond to topics and columns correspond to dictionary atoms.
Very small values were thresholded for visualization clarity.
Different atoms capture different prediction patterns;
for example, atom 5 assigns a highly positive weight to the \texttt{[kid, child, disney, family]} topic and down-weighs \texttt{[sexual, violence, nudity, sex]}, while atom 11 acts in an opposite manner.
Given the context of the review, CEN combines just a few atoms to make a prediction.}
\label{fig:imdb-dict-tpc}
\end{figure}


==> figures/imdb-plots.tex <==
%!TEX root = ../paper.tex

\begin{figure}[t!]
    \centering
    \includegraphics[width=\textwidth]{topic_histograms.pdf}
    \caption{%
    Histograms of test weights assigned by CEN to 6 topics: Acting- and plot-related topics (upper charts), genre topics (bottom charts).
    Note that acting-related topics are often bi-modal, i.e., contributing either positive, negative, or zero weight to the sentiment prediction in different contexts.
    Genre topics almost always have negligible contributions.
    This allows us to conclude that the learned model does not have any particular biases towards or against any a given genre.}
    \label{fig:imdb-dict-hist}
\end{figure}


==> figures/mnist-plots.tex <==
%!TEX root = ../paper.tex

\begin{figure}[b]
    \centering
    \includegraphics[width=\textwidth]{mnist-preds-qualitative}
    \caption{%
    Visualization of the top 3 prediction explanations provided by the CEN model for correctly classified (left), misclassified (middle), and adversarial (right) digits.
    Adversarial examples were generated using the fast gradient sign method (FGSM)~\cite{papernot2016practical}.}
    \label{fig:mnist-plots}
\end{figure}


==> figures/survival.tex <==
%!TEX root = ../paper.tex

\begin{figure}[th!]
\centering
\begin{tikzpicture}
    % Redefine some styles
    \tikzstyle{latent} = [circle,fill=white,draw=black,inner sep=1pt,
    minimum size=17pt, font=\fontsize{9}{9}\selectfont, node distance=1]

    \node (x1) [obs] {$\cv^1$};
    \node (x2) [obs, right=14pt of x1] {$\cv^2$};
    \node (x3) [obs, right=14pt of x2] {$\cv^3$};
    \node (x_) [obs, transparent, right=10pt of x3] {};


    \node (h1) [det, above=10pt of x1] {$h^1$};
    \node (h2) [det, right=10pt of h1] {$h^2$};
    \node (h3) [det, right=10pt of h2] {$h^3$};

    \node (h4) [det, right=10pt of h3] {$h^4$};
    \node (h5) [det, right=10pt of h4] {$h^5$};
    \node (h6) [det, right=10pt of h5] {$h^6$};

    \edge {x1} {h1};
    \edge {x2} {h2};
    \edge {x3} {h3};

    \edge {h1} {h2};
    \edge {h2} {h3};
    \edge {h3} {h4};
    \edge {h4} {h5};
    \edge {h5} {h6};

    \node (th1) [latent, above=10pt of h4] {$\theta^1$};
    \node (th2) [latent, above=10pt of h5] {$\theta^2$};
    \node (th3) [latent, above=10pt of h6] {$\theta^3$};

    \edge {h4} {th1};
    \edge {h5} {th2};
    \edge {h6} {th3};

    \node (y1) [obs, above=10pt of th1] {$y^1$};
    \node (y2) [obs, above=10pt of th2] {$y^2$};
    \node (y3) [obs, above=10pt of th3] {$y^3$};

    \edge {th1} {y1};
    \edge {th2} {y2};
    \edge {th3} {y3};

    \edge[-] {y1} {y2};
    \edge[-] {y2} {y3};

    \node (z) [obs, above=37pt of h2] {$\xv$};

    \edge {z} {y1};
    \edge[bend left=25] {z} {y2};
    \edge[bend left=25] {z} {y3};

    % \plate {CIM} {(h1)(h6)(x3)} {Contextualization};
\end{tikzpicture}
\caption{%
CRF-based CIM for survival analysis.
LSTM is used to embed the context, approximate the dynamics of the survival function, and output weights of the attributes for each of the steps.}
\label{fig:CIM-survival}
\vspace{-3ex}
\end{figure}


==> tikzlibrarybayesnet.code.tex <==
% tikzlibrary.code.tex
%
% Copyright 2010-2011 by Laura Dietz
% Copyright 2012 by Jaakko Luttinen
%
% The MIT License
%
% See LICENSE file for more details.

% Load other libraries
\usetikzlibrary{shapes}
\usetikzlibrary{fit}
\usetikzlibrary{chains}
\usetikzlibrary{arrows}

% Latent node
\tikzstyle{latent} = [circle,fill=white,draw=black,inner sep=1pt,
minimum size=20pt, font=\fontsize{10}{10}\selectfont, node distance=1]
% Observed node
\tikzstyle{obs} = [latent,fill=gray!15]
% Constant node
\tikzstyle{const} = [rectangle, inner sep=0pt, node distance=1]
% Factor node
\tikzstyle{factor} = [rectangle, fill=black,minimum size=5pt, inner
sep=0pt, node distance=0.4]
% Deterministic node
\tikzstyle{det} = [latent, diamond]

% Plate node
\tikzstyle{plate} = [draw, rectangle, rounded corners, fit=#1]
% Invisible wrapper node
\tikzstyle{wrap} = [inner sep=0pt, fit=#1]
% Gate
\tikzstyle{gate} = [draw, rectangle, dashed, fit=#1]

% Caption node
\tikzstyle{caption} = [font=\footnotesize, node distance=0] %
\tikzstyle{plate caption} = [caption, node distance=0, inner sep=0pt,
below left=5pt and 0pt of #1.south east] %
\tikzstyle{factor caption} = [caption] %
\tikzstyle{every label} += [caption] %

%\pgfdeclarelayer{b}
%\pgfdeclarelayer{f}
%\pgfsetlayers{b,main,f}

% \factoredge [options] {inputs} {factors} {outputs}
\newcommand{\factoredge}[4][]{ %
  % Connect all nodes #2 to all nodes #4 via all factors #3.
  \foreach \f in {#3} { %
    \foreach \x in {#2} { %
      \path (\x) edge[-,#1] (\f) ; %
      %\draw[-,#1] (\x) edge[-] (\f) ; %
    } ;
    \foreach \y in {#4} { %
      \path (\f) edge[->, >={triangle 45}, #1] (\y) ; %
      %\draw[->,#1] (\f) -- (\y) ; %
    } ;
  } ;
}

% \edge [options] {inputs} {outputs}
\newcommand{\edge}[3][]{ %
  % Connect all nodes #2 to all nodes #3.
  \foreach \x in {#2} { %
    \foreach \y in {#3} { %
      \path (\x) edge [->, >={triangle 45}, #1] (\y) ;%
      %\draw[->,#1] (\x) -- (\y) ;%
    } ;
  } ;
}

% \factor [options] {name} {caption} {inputs} {outputs}
\newcommand{\factor}[5][]{ %
  % Draw the factor node. Use alias to allow empty names.
  \node[factor, label={[name=#2-caption]#3}, name=#2, #1,
  alias=#2-alias] {} ; %
  % Connect all inputs to outputs via this factor
  \factoredge {#4} {#2-alias} {#5} ; %
}

% \plate [options] {name} {fitlist} {caption}
\newcommand{\plate}[4][]{ %
  \node[wrap=#3] (#2-wrap) {}; %
  \node[plate caption=#2-wrap] (#2-caption) {#4}; %
  \node[plate=(#2-wrap)(#2-caption), #1] (#2) {}; %
}

% \gate [options] {name} {fitlist} {inputs}
\newcommand{\gate}[4][]{ %
  \node[gate=#3, name=#2, #1, alias=#2-alias] {}; %
  \foreach \x in {#4} { %
    \draw [-*,thick] (\x) -- (#2-alias); %
  } ;%
}

% \vgate {name} {fitlist-left} {caption-left} {fitlist-right}
% {caption-right} {inputs}
\newcommand{\vgate}[6]{ %
  % Wrap the left and right parts
  \node[wrap=#2] (#1-left) {}; %
  \node[wrap=#4] (#1-right) {}; %
  % Draw the gate
  \node[gate=(#1-left)(#1-right)] (#1) {}; %
  % Add captions
  \node[caption, below left=of #1.north ] (#1-left-caption)
  {#3}; %
  \node[caption, below right=of #1.north ] (#1-right-caption)
  {#5}; %
  % Draw middle separation
  \draw [-, dashed] (#1.north) -- (#1.south); %
  % Draw inputs
  \foreach \x in {#6} { %
    \draw [-*,thick] (\x) -- (#1); %
  } ;%
}

% \hgate {name} {fitlist-top} {caption-top} {fitlist-bottom}
% {caption-bottom} {inputs}
\newcommand{\hgate}[6]{ %
  % Wrap the left and right parts
  \node[wrap=#2] (#1-top) {}; %
  \node[wrap=#4] (#1-bottom) {}; %
  % Draw the gate
  \node[gate=(#1-top)(#1-bottom)] (#1) {}; %
  % Add captions
  \node[caption, above right=of #1.west ] (#1-top-caption)
  {#3}; %
  \node[caption, below right=of #1.west ] (#1-bottom-caption)
  {#5}; %
  % Draw middle separation
  \draw [-, dashed] (#1.west) -- (#1.east); %
  % Draw inputs
  \foreach \x in {#6} { %
    \draw [-*,thick] (\x) -- (#1); %
  } ;%
}

